Preserving Privacy and Utility in LLM-Based Product Recommendations

Large Language Model (LLM)-based recommendation systems leverage powerful language models to generate personalized suggestions by processing user interactions and preferences. Unlike traditional recommendation systems that rely on structured data and collaborative filtering, LLM-based models process textual and contextual information, often using cloud-based infrastructure. This raises privacy concerns, as user data is transmitted to remote servers, increasing the risk of exposure and reducing control over personal information. To address this, we propose a hybrid privacy-preserving recommendation framework which separates sensitive from nonsensitive data and only shares the latter with the cloud to harness LLM-powered recommendations. To restore lost recommendations related to obfuscated sensitive data, we design a de-obfuscation module that reconstructs sensitive recommendations locally. Experiments on real-world e-commerce datasets show that our framework achieves almost the same recommendation utility with a system which shares all data with an LLM, while preserving privacy to a large extend. Compared to obfuscation-only techniques, our approach improves HR@10 scores and category distribution alignment, offering a better balance between privacy and recommendation quality. Furthermore, our method runs efficiently on consumer-grade hardware, making privacy-aware LLM-based recommendation systems practical for real-world use.

==> tables/latency_throughput_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{llllll}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Sequence Length/ Tokens}} & \multicolumn{2}{l}{\textbf{Latency  (s)}} & \multicolumn{2}{l}{\textbf{Throughput (IPS)}} \\ \cline{3-6} 
                                &                                                   & \textbf{GPU}         & \textbf{CPU}        & \textbf{GPU}          & \textbf{CPU}          \\ \hline
\textbf{BERT (Base)}            & 128 tokens (Batch = 20)                           & 0.0872	                    & 0.5762	                   & 133.4	                     & 30.4                     \\ \hline
\textbf{Local LLaMA 1B}         & Entire input as 1 sequence, 1024 tokens           & 7.75                    & 102.64                   & B                     & B                     \\ \hline
\textbf{Global LLM APLI}        & Entire input as 1 sequence, 2048 tokens           & 2.74                    & 2.74                   & C                     & C                     \\ \hline
\end{tabular}
\caption{}
\label{tab:latency-throughput}
\end{table*}

